Fair Byzantine Agreements for Blockchains

Byzantine general problem is the core problem of the consensus algorithm, and many protocols are proposed recently to improve the decentralization level, the performance and the security of the blockchain. There are two challenging issues when the blockchain is operating in practice. First, the outcomes of the consensus algorithm are usually related to the incentive model, so whether each participant's value has an equal probability of being chosen becomes essential. However, the issues of fairness are not captured in the traditional security definition of Byzantine agreement. Second, the blockchain should be resistant to network failures, such as cloud services shut down or malicious attack, while remains the high performance most of the time. This paper has two main contributions. First, we propose a novel notion called fair validity for Byzantine agreement. Intuitively, fair validity lower-bounds the expected numbers that honest nodes' values being decided if the protocol is executed many times. However, we also show that any Byzantine agreement could not achieve fair validity in an asynchronous network, so we focus on synchronous protocols. This leads to our second contribution: we propose a fair, responsive and partition-resilient Byzantine agreement protocol tolerating up to 1/3 corruptions. Fairness means that our protocol achieves fair validity. Responsiveness means that the termination time only depends on the actual network delay instead of depending on any pre-determined time bound. Partition-resilience means that the safety still holds even if the network is partitioned, and the termination will hold if the partition is resolved.

==> outline.tex <==
sec.1 intro
BA
why define fair
 - for blockchain
 - novel concept for BA
useful properties of BA for blockchain
 - responsive
 - async secure
 
contribution
  1. fair
  2. fair thm (thm 0)
  3. FAS BA
  4. FAS BA is practical (thm1, thm2)
  5. experiment on FAS BA
  
Related work



Technical overview
  1. RBA (why AS)
  2. HBA (why Responsive)
  

sec.2 Model

sec.3 RBA
A) protocol
B) Agreement
C) Termination


sec.4 HBA
A) protocol
B) Agreement
C) Termination
D) Responsiveness


sec.5 Exp
A) Responsiveness
B) partition-tolerance

sec.6 more discussion
